Tight Competitive Ratios of Classic Matching Algorithms in the Fully Online Model

Huang et al.~(STOC 2018) introduced the fully online matching problem, a generalization of the classic online bipartite matching problem in that it allows all vertices to arrive online and considers general graphs. They showed that the ranking algorithm by Karp et al.~(STOC 1990) is strictly better than $0.5$-competitive and the problem is strictly harder than the online bipartite matching problem in that no algorithms can be $(1-1/e)$-competitive. This paper pins down two tight competitive ratios of classic algorithms for the fully online matching problem. For the fractional version of the problem, we show that a natural instantiation of the water-filling algorithm is $2-\sqrt{2} \approx 0.585$-competitive, together with a matching hardness result. Interestingly, our hardness result applies to arbitrary algorithms in the edge-arrival models of the online matching problem, improving the state-of-art $\frac{1}{1+\ln 2} \approx 0.5906$ upper bound. For integral algorithms, we show a tight competitive ratio of $\approx 0.567$ for the ranking algorithm on bipartite graphs, matching a hardness result by Huang et al. (STOC 2018).

==> hardness.tex <==
\section{Problem Hardness}  \label{sec:problem_hardness}

In this section, we generalize the hard instance for \wtf and prove that no (randomized) algorithm can be better than $(2-\sqrt{2})$-competitive for \fofmp, even on bipartite graphs.

We first explain the difficulty for constructing a hard instance for arbitrary algorithms.
Consider the hard instance from Section~\ref{sec:wtfhardness}.
Since for all $t\geq 2$, the vertices in $U_t$ are all neighbors of $u_{t-1,1}$, we know that at the deadline of $u_{t,1}$ (which is after the deadline of $u_{t-1,1}$), all vertices in $U_t$ are completely revealed (refer to Figure~\ref{figure:u21ddl}).
Further, $u_{t, 1}$ has edges to all vertices in $V_t$.
Consequently, all edges between $U_t$ and $V_t$ are revealed.
Hence, a smart algorithm can easily match every $u_{t,i}$ to $v_{t,i}$ at its deadline and give a perfect matching.

\begin{figure}[!h]
	\centering
	\resizebox*{45mm}{!}{
		\begin{tikzpicture}
		[font=\bf,line width=0.3mm,scale=.8,auto=left,every node/.style={circle,draw}]
		\tikzset{deadline/.style={red,line width=0.7mm}}
		\def \n {4}
		\node at (1,1.4*\n+0.5) (prev) {\LARGE $U_1$};
		\foreach \i in {1,...,\n}
		{
			\ifthenelse{\i = 1}{\node[deadline] at (1,1.4*\n-1.4*\i) (u\i) {$u_{2,\i}$};}{\node at (1,1.4*\n-1.4*\i) (u\i) {$u_{2,\i}$};}
			
		};
		\foreach \i in {1,...,\n}
		{
			\node at (6,1.4*\n-1.4*\i) (v\i) {$v_{2,\i}$};
			\foreach \j in {1,...,\i}
			{
				\ifthenelse{\j = 1}{\draw[deadline] (u\j) to (v\i);}{\draw (u\j) to (v\i);}
				
			};
		};
		\node at (1,-1.4-0.5) (uu1) {\LARGE $U_3$};
		% \draw (prevv) to (prev);
		\foreach \i in {1,...,\n}
		{
			\draw[out=135,in=225] (u\i) to (prev);
			\ifthenelse{\i = 1}{\draw[deadline,out=135,in=225] (uu1) to (u\i);}{\draw[out=135,in=225] (uu1) to (u\i);}
			
		};
		\end{tikzpicture}
	}
	\caption{At the deadline of $u_{2,1}$, $v_{2,1}$ has less neighbor than $v_{2,2},v_{2,3},v_{2,4}$.}
	\label{figure:u21ddl}
\end{figure}


Intuitively, we would like to delay the arrivals of some vertices in $U_t$ (e.g., $u_{2,2}$, $u_{2, 3}$, and $u_{2, 4}$ in Figure~\ref{figure:u21ddl}) so that at $u_{t,i}$'s deadline, $v_{t,i}$ is indistinguishable from other available neighbors of $u_{t, i}$ in $N(u_{t,i})$. 
If this can be done, the best an algorithm can do is to mimic \wtf, i.e., to match the remaining portion of $u_{t,i}$ uniformly to all available neighbors $v \in N(u_{t,i})$.

In this section, we construct a new instance that inherits the graph structure of the previous hard instance from Section~\ref{sec:wtfhardness}, but reveals the graph gradually to the algorithm so that for each vertex $u$, all vertices in $N(u)$ are indistinguishable at $u$'s deadline.
In particular, we will guarantee that all vertices in $N(u)$ have the same set of neighbors.
Then, we randomly assign the identities of these neighbors and prove that no matter which algorithm is used, in expectation, the water-level of all available neighbors of $u$ will get a uniform increment. 
This property is then sufficient for deriving a $(2-\sqrt{2})$ upper bound on the competitive ratio of the algorithm.


\paragraph{Structure of the Hard Instance.}

We first describe the graph structure of the hard instance as well as the deadlines of the vertices, deferring the discussion on the standard trick of randomly assigning identities of vertices to the proof of the problem hardness.

At a high-level, we run $L$ copies of the hard instance for \wtf from Section~\ref{sec:wtfhardness} simultaneously.
We label the vertices by $u_{t,i,l}$ and $v_{t,i,l}$, where $t\in[m]$, $i\in[k]$, and $l\in[L]$.
Again, we group the vertices into disjoint sets. 
For any $t\in[m]$, and any $l\in[L]$, let $U_{t,l} = \{ u_{t,1,l},\ldots,u_{t,k,l} \}$ and $V_{t,l} = \{ v_{t,1,l},\ldots,v_{t,k,l} \}$.
For the internal edges within the same group, we will keep the same upper triangle graph between $U_{t, l}$ and $V_{t, l}$ as in the previous construction.
The external edges that connect vertices from different groups, however, require some subtle changes.
Instead of simply connecting vertices in $U_{t, l}$'s with those in $U_{t+1, l}$'s with a set of the $h$-induced edges between them, we will instead connects $U_{t, l}$ with a shifted version of $U_{t+1, l}$ defined as follows. 
%However, instead of connecting $U_{t, l}$'s to the next 
%The key difference from instance and the algorithm hard instance is that, we give another partition of the $u$ vertices, which is used to define the $h$-induced edges.
For all $t\in[m-1],l\in[L]$, define $\widehat{U}_{t+1,l} = \{ u_{t+1,j,l-k^{t-1}(j-1)} : j\in[k] \}$ (see Figure~\ref{figure:problemhardness}).
Due to the third index $l-k^{t-1}(j-1)$, we create some extra dummy vertices with non-positive indexes (in the third index).
However, it is easy to see that the number of dummy vertices is at most $O(m\cdot k^{m+1})$, which is independent of $L$.

In sum, there are two types of edges in the graph:
\begin{enumerate}
	\item Upper triangle edges between $U_{t,l}$ and $V_{t,l}$: $\forall t\in [m], i\in[k], l\in[L]$ and $j\geq i$, $(u_{t,i,l},v_{t,j,l})\in E$;
	
	\item $h$-induced edges between $U_{t,l}$ and $\widehat{U}_{t+1,l}$: create a subgraph $H$ between $U_{t,l}$ and $\widehat{U}_{t+1,l}$. In particular, regard $u_{t,i,l}$ as $u_{t,i}$ and $u_{t+1,j,l-k^{t-1}(j-1)}$ as $u_{t+1,j}$, as in Section~\ref{sec:wtfhardness}. \zhiyi{please add a formal definition here.}
\end{enumerate}

\begin{figure}[htp]
	\centering
	\resizebox*{100mm}{!}
	{
		\begin{tikzpicture}
		[font=\bf,line width=0.5mm,scale=.8,auto=left,every node/.style={circle,draw}]
		\tikzset{deadline/.append style={red,line width=1mm}}
		\usetikzlibrary{shapes,fit}
		\def \n {3}
		\def \X {7}
		\foreach \l in {1,...,3}
		{
			\foreach \x in {1,...,\X}
			{
				\foreach \i in {1,...,\n}
				{
					\def \delta {2.5}
					\def \px {1+\x*5-5}
					\def \py {\delta*2*\n-\delta*\n*\l+\delta*\n-\delta*\i}
					\def \su {\x+\i}
					\node at (\px,\py) (u\l\i\x) {$u_{\l,\i,\x}$};
				}; 
			}
		}
		\node[dashed, line width=1mm, rectangle, fit=(u113) (u123) (u133)](can) {\Huge $\qquad {U}_{1,3}$};
		\node[dashed, line width=1mm, rectangle, fit=(u114) (u124) (u134)](can) {\Huge $\qquad {U}_{1,4}$};
		\node[dashed, line width=1mm, rectangle, fit=(u115) (u125) (u135)](can) {\Huge $\qquad {U}_{1,5}$};
		\node[dashed, line width=1mm, rectangle, fit=(u116) (u126) (u136)](can) {\Huge $\qquad {U}_{1,6}$};
		\node[dashed, line width=1mm, rectangle, fit=(u117) (u127) (u137)](can) {\Huge $\qquad {U}_{1,7}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=27, fit=(u213) (u222) (u231)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{2,3}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=27, fit=(u214) (u223) (u232)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{2,4}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=27, fit=(u215) (u224) (u233)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{2,5}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=27, fit=(u216) (u225) (u234)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{2,6}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=27, fit=(u217) (u226) (u235)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{2,7}$};
		\node[dashed, line width=1mm, rectangle,rotate fit=9.5, fit=(u317) (u324) (u331)](can) {\Huge \null\\ $\qquad\qquad \widehat{U}_{3,7}$};
		\end{tikzpicture}
	} 
	\caption{Part of the problem hard instance: illustrating example with $k=3$.}
	\label{figure:problemhardness}
\end{figure}

Note that the hard instance is bipartite, where one side of the vertices are $\bigcup_{\text{odd } t, i\in[k], l\in[L]}U_{t,i,l} \cup \bigcup_{\text{even } t, i\in[k], l\in[L]}V_{t,i,l}$ and the other side has the remaining.

Finally, we define the deadlines of the $u$ vertices. For each vertex $u_{t,i,l}$, let $d(t,i,l) \in \mathbb{N}$ denote its deadline, where $d$ is a function to be specified below. 
After the latest deadline among $u$ vertices, let the deadlines of $v$ vertices be reached. Again, the relative order of $v$ vertices do not matter. We do not explicitly specify the arrivals of vertices. Instead, let the arrival of a vertex be right before the earliest deadline among its neighbors (including itself).

Let the deadline function be defined as $d(t,i,l) \eqdef k^{t-3} + i \cdot k^{t-2} + l$.
It is easy to check that for every fixed $l\in[L]$, the deadlines of $u_{t,i}$ follow the lexicographical order of $(t,i)$, just as in our algorithm hard instance from Section~\ref{sec:wtfhardness}.
Next, we show that vertices in $U_{t,l}$ have earlier deadlines than vertices in $\widehat{U}_{t+1,l}$.
For any $i,j\in[k]$, we have
\begin{align*}
d(t+1,j,l-k^{t-1}(j-1)) & = k^{t-2} + j \cdot k^{t-1} + l-k^{t-1}(j-1) = k^{t-2} + k^{t-1} + l \\
& > k^{t-3} + k\cdot k^{t-2} + l = d(t,k,l) > d(t,i,l).
\end{align*}

\begin{lemma} \label{lemma:indistinguishable}
	At $d(t,i,l)$, all vertices in $N(u_{t,i,l})$ have the same set of neighbors.
\end{lemma}
\begin{proof}
Fix arbitrary $t\in[m-1]$ and $l\in[L]$.
Observe that we have
\begin{equation*}
	N(u_{t,k,l}) \subsetneq \ldots \subsetneq N(u_{t,2,l}) \subsetneq N(u_{t,1,l}) = V_{t,l} \cup \widehat{U}_{t+1,l}.
\end{equation*}
 
 
 
 For each $u_{t,i,l}$, where $t\geq 2$, let $l_i=l+k^{t-2}(i-1)$ be the index such that $u_{t,i,l} \in \widehat{U}_{t,l_i}$.
 
 $d(t,i,l) < d(t-1, 1, l+k^{t-2}\cdot i), \quad \forall t>1, i<k$.
 
Moreover, all vertices in $N(u_{t,1,l})$ arrive right before $d(t,1,l)$.
By the graph structure, to show that all vertices in $N(u_{t,i,l})$ are indistinguishable,
it suffices to show that at $d(t,i,l)$, all vertices $\{u_{t,j,l}: j>i\}$ have not arrived.

By our construction, $u_{t,j,l}\in \widehat{U}_{t,l_j}$ arrives at the earliest deadline among vertices in $U_{t-1,l_j}$, which is $d(t-1,1,l_j)$, by the first inequality. Thus for all $j>i$, we have
\[
\text{Arrival of } u_{t,j,l} = d(t-1,1,l_j) \geq d(t-1,1,l_{i+1}) = d(t-1, 1, l+k^{t-2}\cdot i) > d(t,i,l),
\]
where the last inequality follows from the third inequality stated above.
\end{proof}

Now we are ready to prove the main theorem.
\begin{theorem}\label{theorem:problem_hardness}
	No algorithm can do better than $(2-\sqrt{2})$-competitive for \fofmp, even on bipartite graphs.
\end{theorem}
\begin{proof}
%	\zhihao{elaborate more about the following sentence.}
Equipped with the indistinguishability property from Lemma~\ref{lemma:indistinguishable},
for any algorithm, after the deadline of every $u_{t,i,l}$, we can randomly assign the identities of vertices in $N(u_{t,i,l})$
such that in expectation, the water levels of all available neighbors of $u_{t,i,l}$ get a uniform increment.

Therefore, if in the algorithm, the water level of every $u_{t,i,l}$ reaches $1$ after its own deadline, then following exactly the same analysis as in Section~\ref{sec:wtfhardness}, we conclude that the algorithm must have the same performance as the \wtf algorithm in expectation.

%consider the family of random instances that uniform randomly assigning identities to the neighbors $N(u_{t,i,l})$ in future rounds.
%Moreover, the water level of $u_{t,i,l}$ is ``prepared'' before $d(t,i,l)$ as running \wtf in the hard instance from Section~\ref{sec:wtfhardness}.
%Indeed, $d(t,i,l) > d(t-1,m,l_i)$ by the second inequality of Lemma~\ref{lemma:indistinguishable}, where $l_i=l+k^{t-2}(i-1)$ is the index such that $u_{t,i,l} \in \widehat{U}_{t-1, l_i}$.


Some complication arises when the water level of some $u = u_{t,i,l}$ is not $1$, after its own deadline.
Indeed, an algorithm might decide to leave $u$ unmatched.
Or, under some (random) realization, the water levels of all available neighbors of $u$ reach $1$ and thus $u$ cannot be matched.
However, our random instances guarantee that in expectation (over the randomness of the algorithm and instances simultaneously), the increment of water levels of $N(u)$ are always uniformly distributed. This leaves us to consider a modified version of \wtf that may leave some $u$ vertices partially matched.
%but chooses the vertex with lowest water level when it decides to match.
We give the complete proof in Appendix~\ref{appendix:modified}.

Recall that we create $O(m\cdot k^{m+1})$ vertices in the instance that could potentially increase \opt. However, by setting $L$ sufficiently large, this quantity becomes negligible and our hardness ratio tends to the same ratio $(2-\sqrt{2})$ as in Section~\ref{sec:wtfhardness}.
\end{proof}

The above hard instance directly applies to several other online matching models. We provide the formal definitions of these models and the complete proof in Appendix~\ref{app:hard_other}.
\begin{corollary}
	\label{cor:hard_other}
	No algorithm can do better than $(2-\sqrt{2})$-competitive for \textsf{Online Preemptive Matching}, \textsf{Online Edge-arrival Matching} and \textsf{Two-sided Online Matching~\cite{icalp/WangW15}}, even if fractional matching is allowed.
\end{corollary}




% Thus, we only pay attention to the critical vertices. At first, We introduce a relaxed version of the problem, in which we remove all the constraints $x_{uv} \geq 0$ and the constraints $\sum_{v:(u,v)\in E} {x_{uv}} \leq 1$ for all RHS vertices. Then for any algorithm for the original problem, we modify it to an algorithm for the relaxed problem. That is: at the deadline of an LHS vertex $u$, we first simulate the original algorithm, and then if $\sum_{v:(u,v)\in E} {x_{uv}} \neq 1$, we arbitrary choose a neighbor $v$ and let $x_{uv} = x_{uv} + 1 - \sum_{v:(u,v)\in E} {x_{uv}}$. Comparing the modified algorithm to the original one, we have that for any edge, if the water flow decrease, there must exist a related LHS vertex $u$, whose water-level exceed 1 at that time. Because the water of any vertex $w_u$ can't exceed 1 in the original algorithm, so that the decreased amount $\Delta^- = w_u+\Delta^+ -1$ is no larger than the increase of the flow-in edge $\Delta^+$. Thus, the modified algorithm can not be worse than the original one.

% Next, we can use a similar analysis as the one in the algorithm hardness section. Let $\tau(x)$ be the passive expected water level of a $x\cdot k-th$ LHS vertex in one group at its deadline. Because in the hard instance, all the neighbors of any critical LHS vertices are uniformly randomly assigned, so at the deadline of an $x\cdot k-th$ LHS vertex, the expected water level of its neighbor will uniformly increase the amount $\frac{1-y}{1-f(y)+f(c-y)}$. Thus, we get that for any $x\in(0,1]$, the water level of its neighbor is $\frac{1-y}{1-f(y)+f(c-y)} = c-\tau(x)$, which means the passive water level of every $u_i,v_i$ pair is c, and the algorithm solution is $c\cdot n$.

%\begin{theorem}\label{theorem:problem_hardness}
%	No algorithm has a competitive ratio strictly larger than $2-\sqrt{2}$ for \fobmp.
%\end{theorem}
%\begin{proof}
%	For the optimal side, we can at least pair all critical LHS vertices with their perfect partner. Hence, we have that $\textbf{OPT} \geq mk\cdot T$.
%	
%	In the algorithm side, If we consider the expectation and only focus on the critical LHS vertices and their perfect partner, We can easily follow the similar proof as that in Theorem~\ref{the:wthard} and get that the expected performance on the critical vertices and their perfect partner of the modified algorithm is $E(\alg') = (2-\sqrt{2})\cdot mk\cdot T$. Thus, the overall expected performance $E(\alg') \leq (2-\sqrt{2})\cdot mk\cdot T + mk\cdot m^k$. Furthermore, we can bound any algorithm by $\alg \leq \alg' \leq ((2-\sqrt{2})\cdot + \frac{m^k}{T})\cdot OPT$. Notice that we can set $T>>m^k$, which implies no algorithm has a competitive ratio strictly larger than $2-\sqrt{2}$ for the \fomp, even in the fractional version and restricted to bipartite graph.
%\end{proof}
